AWA: Adversarial Website Adaptation

One of the most important obligations of privacy-enhancing technologies is to bring confidentiality and privacy to users' browsing activities on the Internet. The website fingerprinting attack enables a local passive eavesdropper to predict the target user's browsing activities even she uses anonymous technologies, such as VPNs, IPsec, and Tor. Recently, the growth of deep learning empowers adversaries to conduct the website fingerprinting attack with higher accuracy. In this paper, we propose a new defense against website fingerprinting attack using adversarial deep learning approaches called Adversarial Website Adaptation (AWA). AWA creates a transformer set in each run so that each website has a unique transformer. Each transformer generates adversarial traces to evade the adversary's classifier. AWA has two versions, including Universal AWA (UAWA) and Non-Universal AWA (NUAWA). Unlike NUAWA, there is no need to access the entire trace of a website in order to generate an adversarial trace in UAWA. We accommodate secret random elements in the training phase of transformers in order for AWA to generate various sets of transformers in each run. We run AWA several times and create multiple sets of transformers. If an adversary and a target user select different sets of transformers, the accuracy of adversary's classifier is almost 19.52% and 31.94% with almost 22.28% and 26.28% bandwidth overhead in UAWA and NUAWA, respectively. If a more powerful adversary generates adversarial traces through multiple sets of transformers and trains a classifier on them, the accuracy of adversary's classifier is almost 49.10% and 25.93% with almost 62.52% and 64.33% bandwidth overhead in UAWA and NUAW, respectively.

==> content/NUAWA.tex <==
We run AWA five times and generate five sets of generators which each one consists of 95 generators.

==> content/old_background.tex <==
More than two million daily users take advantage of The Onion Router (TOR) services[1i], among which anonymity and protection from eavesdroppings are two of the most prominent. Different kinds of research have been conducted previously to breach the TOR's privacy feature it provides for its users[3, 10, 5, 6, 7, 8i]. Website Fingerprinting is one such type of traffic analysis attack which by extracting traffic patterns from the visited website, can form a unique fingerprint of acquired traffic flow, and undermine TOR's protection by detecting the website that the user has been just visiting[7, 13, 15, 25, 26, 37, 38D].

\subsection{Website Fingerprinting}
Three entities play key roles in the threat model of the website fingerprinting attack, Adversary, user, and Privacy-Enhancing Technologies (PETs), e.g., TOR. A user utilizes PET to keep his/her link to confidential and anonymous. Since most of PETs are publicly available, an adversary can use them to generate a set of network traffic from his/her favorite website and train a classifier on them to predict the browsing activity of users. It is notable that since an adversary has no access to the label of network traffic generated by the target user, s/he only can evaluate the performance of his/her classifier on the network traffic being generated by him/her.

Two initial presumptions are taken for the attacker in WF scenarios. First, the attacker is local, which means (s)he is located somewhere between the TOR client and the TOR bridge in the network where he can access the link in between. Second, the attacker is passive, meaning that he could only capture the ongoing packets and is not allowed to manipulate, drop, delay, or insert any of them. Any potential eavesdropper whose features conforms to what mentioned can play the role of the attacker (e.g., Autonomous Systems (AS), Internet Service Providers (ISP), and network administrators). The attacker is also considered to be aware of the client's identity (figure 1 depicts the threat model and attacking scenario).

For the attack to be carried out, the attacker first needs to capture a set of traffic traces while visiting a collection of websites, notably those that he is interested in detecting. Thereafter, some unique features shall be extracted from each trace that helps each website become conspicuous to classifiers, amongst other websites. One can find loads of such features in WF literature through previous studies (e.g., packet size [25i], time and volume [36i], edit-distance score [28i], rate of traffic bursts in both directions [9i]). By doing so, the attacker could attain several feature vectors that are used to train his supervised classifier. A common assumption made by previous studies is that attackers can parse the web traffic generated by visiting a website, and he can isolate it from other kinds of traffic on the net. Similar to prior works, we assume that parsing is not needed or has been done beforehand. 

A struggle which the attacker is confronted with is that (s)he can not capture and keep track of traffic traces for all websites on the web, and the number of websites of which he can record the traffic traces is not infinite. Therefore, the attacker identifies several websites (s)he is interested in monitoring, and the scope of the attack is bounded to the detection of this monitored set. All other websites which reside out of this scope are attributed to an unmonitored set. With respect to this constraint, there are two scenarios to evaluate WF attacks and defenses: closed-world scenario and open-world scenario.

The closed-world scenario assumes that the client only visits the websites belonging to the monitored set, and the attacker also uses the samples from the monitored set for his training and testing process. The closed-world scenario consists of ideal settings for the attacker and thus does not show the real-world performance of him. On the other hand, defeating the attacker in this scenario would be considered as overcoming him in his most advantageous situation. 
There is a more realistic scenario (open-world scenario) in which the client is free to visit the websites from both monitored and unmonitored set. In this scenario, the attacker trains his classifier using monitored set samples as well as some samples from the unmonitored set. Then in the test phase, the classifier is evaluated against both monitored and unmonitored traces while unmonitored traces are picked up from remaining samples on which it had not been trained. 

%\subsection{Threat Model}
%Three entities play key roles in the threat model of the website fingerprinting attack, Adversary, user, and Privacy-Enhancing Technologies (PETs), e.g., TOR. A user utilizes PET to keep his/her link to confidential and anonymous. Since most of PETs are publicly available, an adversary can use them to generate a set of network traffic from his/her favorite website and train a classifier on them to predict the browsing activity of users. It is notable that since an adversary has no access to the label of network traffic generated by the target user, s/he only can evaluate the performance of his/her classifier on the network traffic being generated by him/her.
%An essential point about any defense mechanism being implemented on PETs is that an adversary has access to network traffic of every implemented method in PETs to defend against website fingerprinting attacks. We focus on adversarial example generating methods in this paper. If TOR implements adversarial example methods such as FGSM or Carlini on network traffic to cause the adversary's classifier to predict incorrectly, an adversary can generate network traffic for different websites by TOR and train a classifier on them. In the context of adversarial machine learning, training on adversarial examples is one of the most effective defenses against adversarial example attacks. Therefore, when an adversary trains a classifier on the network traffic being perturbed based on an adversarial example algorithm, s/he is doing adversarial training, and his/her classifier becomes more robust against adversarial example attack which has been implemented on PETs. Hence adversarial example being implemented on TOR loos its effectiveness. Accordingly, adversarial training is a part of the threat model of website fingerprinting attack, and we need an adversarial example generating method which is more resistant against adversarial training.

\subsection{Website Trace Representation}
Each trace of a website is a sequence of packets direction in the order that they are received. This trace is called Direction Sequence (DS). For $DS^i$, we have:
\begin{equation}
\begin{split}
& DS^i =\; <d^i_1, d^i_2, ..., d^i_n> , \\
& s.t. \quad d^i_j \in \{+1,-1\},\\
\end{split}
\end{equation}
where $d^i_j$ is the $j^{th}$ packet direction of trace $i$. The direction of packets from the client to the server is $+1$ and from the server to the client is $-1$.
We consider each website trace as a Burst Sequence (BS) to simplify making perturbation for each trace. Burst is a sequence of Consecutive packets which all have the same direction. BS is a sequence of burst size multiplied to burst direction. All packets in a burst have the same direction, which is equal to burst direction. For $BS^i$, we have:

\begin{equation}
\begin{split}
& BS^i =\; <|B^i_1| \times D^i_1, |B^i_2| \times D^i_2, ..., |B^i_m| \times D^i_m>, \\ s.t. \quad B^i_j = < d^j_1, d^j_{2}, ..., d^j_{l}>,  &\:D^i_j \in \{+1,-1\}, \:d^j_k = D^i_j,  D^i_{p} = -1 \times D^i_{p-1},\: k \in [1,l],\: j \in [1,m],\: p \in (2,m]
\end{split}
\end{equation}

where $B^i_j$ is the $j^{th}$ burst of $BS^i$, and the $D^i_j$ is the direction of this burst, which is the same as all packets in $B^i_j$. The order of packets direction in $DS^i$ and $BS^i$ are the same. 

\subsection{Deep Neural Networks}
Deep neural networks (DNN) are multi-layer functions that receive $x_i \in \mathcal{X}$ as input and outputs $y_i = f_{DNN}(x_i)$ ($y_i \in \mathcal{Y}$). Three important DNNs which are mostly used in network traffic classification are Convolutional Neural Networks (CNN), Recurrent Neural Networks (RNN), and Stacked Denoising Autoencoders (SDAE). DNNs are revealed to have high performance on raw data extracted from network traffic and do not need manual feature engineerings to reach high accuracies, Amongst which, One-Dimensional Convolutional Neural Network (1D-CNN) has got the best results in network traffic classification tasks[7, 8, 10, 17 AWA]. 
A neural network consists of three parts: an input layer, a bunch of hidden layers inside, and an output layer. Each layer includes a set of neurons with non-linear activation functions and parameters (weights and biases) related to them. For the act of labeling, there exist $k$ labels for an input $x$ where it gets the label $\hat{y} = \underset{0\leq i<k}{\mathrm{argmax}}\,f_{DNN}(x)_i$ from the model function. During the training phase, the optimum values for the network parameters are calculated so that the loss function $J$, which indicates the distance between actual and predicted labels, will be minimized:
\begin{equation}
\theta^{*} = \underset{\theta}{\mathrm{argmin}} \; J(\theta, x, y)
\end{equation}.
This is usually done using some common versions of the gradient descent algorithm.

\subsection{Adversarial Example}
In spite of their remarkable achievements and high performances in complicated tasks, DNNs have been demonstrated to have a critical vulnerability. Adversarial examples are intentionally crafted inputs, which cause the victim classifier to make a mistake about the correct label of the input. Considering $f^*$ as a classifier that always designates the correct label with 100\% probability, we define adversarial example $x'$ as:
\begin{equation} 
\begin{split}
&f^*(x') = y,\\
&f(x') = y',\quad s.t.\: y'\, \neq y\\
\end{split}
\end{equation}.
To create an adversarial example $x'$, one should add the perturbation vector $\xi$ to the real input $x$ like: $x' = x + \xi$. After crafting the $x'$, the actual class of $x'$ and $x$ should be the same. To calculate the optimal perturbation, one should remember that the amount of perturbation should be limited to a specific bound (here $L_p = \left\lVert x'-x\right\rVert_p$) since it is obvious that a large amount of perturbation or noise could easily change the class of data. With that said, the adversarial example generating process could be formulated as follow:
\begin{equation}
\begin{split}
\label{AE_MP}
& \underset{x'}{\mathrm{argmin}} \;\left\lVert x' - x \right\rVert_p\\
s.t.\: & f^*(x') = y, f(x') = y', y' \neq y, x' \in Domain(x)
\end{split}
\end{equation}.
Adversarial example constructed by mentioned conditions is called untargeted since it would be misclassified to any class other than the real one. Otherwise, if we want our crafted example $x'$ to cause the model to misclassify it to an exact target class $t$ ($y'=t$), then we call it a targeted adversarial example.
Several methods have been introduced to generate adversarial examples so far, of which Goodfellow et al. [14 ANT] and Carlini et al. [8m] are two popular ones. Goodfellow et al. proposed a fast gradient sign method (FGSM) whose idea is to create an untargeted adversarial example by moving toward the gradient of the model's loss function. the perturbation is calculated through the equation:
\begin{equation}
\begin{split}
\xi = \epsilon. sign(\nabla_x J(\theta, x, y))
\end{split}
\end{equation},
where $\nabla_x J(\theta, x, y)$ is the gradient of the loss function w.r.t. an input $x$ and $\epsilon$ tends to control the amplitude of perturbation.
Carlini et al. [8m] proposed another efficacious method for generating  adversarial examples formulated as follow:
\begin{equation}
\begin{split}
& min \left \| \xi \right \|_{p} + c\cdot g(x+\xi),\\
& s.t. x + \xi \in [0,1]^{n}
\end{split}
\end{equation}
where it tries to find the fine $\xi$, which can succeed in minimizing the objective function $g(x+\xi)$ and the $L_{p}-norm$ distance metric (including $l_{0}, l_{2}, and l_{\infty}$). $c$ is a constant parameter to tune the proper ratio between distance metric and objective function and could be obtained by doing a binary search. Multiple objective functions had been examined, and two were chosen for the targeted and untargeted attack, respectively. For the target class $t$ the objective function would be:
\begin{equation}
\begin{split}
& g(x') = \underset{i \neq t}{max}(f(x')_{i}) - f(x')_{t},
\end{split}
\end{equation}
and for untargeted attack having the $y$ as a real class we have:
\begin{equation}
\begin{split}
& g(x') = f(x')_{y} - \underset{i \neq y}{max}(f(x')_{i}),
\end{split}
\end{equation}
as the objective function.  
Moosavi-Dezfooli et al. [33 nasr] also proposed universal adversarial perturbations for the first time where the attacker creates adversarial examples independent of the inputs.



==> content/old_related.tex <==
\subsection{WF Attacks}
before the outbreak of deep learning, most of the studies used to apply manual feature engineering and conventional machine learning classifiers.
The first WF attack was evaluated by Hermann \textit{et al.} [25i], where they reached just 3\% accuracy for the closed world containing 775 websites. Following that, Panchenko \textit{et al.} [26i] achieved an accuracy of 55\% with enhanced extracted features on the same dataset. By using edit-distance, WF attacks gradually improved up to 90\%[27, 28i]. 

Wang \textit{et al.} [36D] proposed the k-NN attack. It utilized a k-nearest neighbor classifier with a combination of features such as the number of bursts, packet ordering, and the number of incoming and outgoing features to measure the similarity between different websites. It achieved a 91\% accuracy in the closed-world setting containing 100 websites and 86\% True Positive Rate (TPR) and 0.6\% False Rate (FPR) in the open-world setting.

Panchenko \textit{et al.} [25D] introduced an attack based on a Support Vector Machine (SVM). Using a cumulative sum of packet length constructed in a particular way, they feed their SVM classifier with the novel feature set. For the closed-world setting, their method achieved 91\% accuracy, and for the open-world setting in a multiclass scenario, they reported 96\% TPR and 9.61\% FPR, respectively.
Hayes and Danezis [13d] suggested a k-fingerprinting attack (k-FP). It extracts the fingerprints of pages by applying a random forest classifier and then feeds the extracted feature vectors to a k-NN classifier. They analyzed and ranked principal features and figured out that the top 20 leading features leak more information about a webpage than the complicated constructed features. The k-FP attack achieved 91\% accuracy for closed-world setting and 88\% TPR and 0.5\% FPR for the open-world setting.

In the following, famous Deep-learning-based WF attacks are explained briefly.
Abe and Goto[2m] introduced the first WF attack employing DNNs. They proposed a Stacked Denoising Autoencoder (SDAE) classifier, and instead of whole handcrafted features that had been used in previous studies, they feed their model just with sequences of raw packet directions. In the sequence, incoming and outgoing packets are represented as "-1" and "+1" values, respectively. Though the team used a deep learning structure for their classifier for the first time, they could not achieve a higher accuracy rate than previous traditional classifiers. They reported an accuracy of 88\% for the closed-world scenario. 

By deploying multiple DNN structures (including SDAE, CNN, and LSTM), Rimer \textit{et al.} [34m] introduced a new set of attacks in their study called Automated Website Fingerprinting (AWF). They also collected a vast dataset of 900 websites with 2500 traces each to increase the effectiveness of their using DNNs. According to the obtained results, their CNN model outperformed others with an accuracy of 96\% for the closed-word scenario.

Following the previous research by Rimer, Sirinam \textit{et al.} [36m] developed a new CNN model classifier which surpassed all previous ones and achieved more than 98\% accuracy in closed-word settings. They collected a dataset of 100 websites with 1000 visits each to evaluate their attack model. Furthermore, their attack model achieved a high accuracy of 90\% against the traffic defended by WTF-PAD [17m] and showed some powerful performance against the one protected by the Walkie-Talkie[39m] method.

\subsection{WF Defenses}
A WF Defense aims to obfuscate the features from which the attacker's model learns to recognize and differentiate traces of each website from those of others. to do so a Defense method should manipulate the traffic sequence, and this work is done by two mainstay techniques: injecting crafted dummy packets and causing delays. The first one is the reason for bandwidth overhead while the latency overhead is dut to the second one. This section will review the most prominent defenses presented so far. 

A few defense methods have been proposed to operate in the application layer. Cherubin \textit{et al.} [11m] proposed two defense techniques ALPaCA and LLaMA in their study. ALPaCA is a serverside method that manipulates the size of different content types within a webpage and tries to make them close to those of average in onion network. With 41\% latency overhead and 44\% bandwidth overhead, respectively, ALPaCA degrades the CUMUL accuracy from 56\% to 33\%. LLaMA is a clientside technique which causes delays to HTTP requests to alter the order of packets. With 9\% latency and 7\% bandwidth overhead, respectively, LLaMA degrades the CUMUL accuracy from 56\% to 34\%.

Some groups of defenses work based on the same constant rate of packets being transmitted. BuFLO [12m] was the first of this kind through which both the client and cooperating node transmit the same size packets with an equal rate. After the page is loaded, a particular amount of time threshold should be elapsed, and the defense process ends. Later, some extended versions of BuFLO were proposed, which tried to improve their predecessor's obscuring power. Tamaraw [6m] keeps transmitting dummy packets until the number of total transmitted bytes reaches or exceeds a fixed parameter. Similarly, CS-BuFLO [ 5m] tried to increase the transmitted bytes up to a power of specific parameter. Even though the BuFLO family achieved satisfying results in defeating different attack manners, they have a very heavy bandwidth and latency overhead. 

By employing the Adaptive Padding method [35m], Juarez \textit{et al.} introduced WTF-PAD [17m]. WTF-PAD tries to obfuscate the inter-arrival time feature by filling the abnormal time gap between two packets of a sequence with dummy ones (average inter-arrival packet times were picked up randomly from a pool of samples gathered from internet normal traffics of websites.) they succeeded to downgrade the k-NN classifier accuracy from 93\% to 17\%. However, Deep fingerprinting [36m] obtained the security of 90\% against WTF-PAD in closed-world settings.
Walkie-Talkie [39m], Supersequence [38m], and Glove [25m] try to use a supersequence method. Supersequence and Glove try to cluster the websites and then estimate a supersequence for each cluster. Then, every traffic trace must be padded so that it becomes similar to the supersequence of the cluster to which it belongs. Walkie-Talkie has two features: Burst-molding and half-duplex communications. All requests and messages should be queued in a buffer and then be sent together so that there is no interference between sent and received messages, and the communication becomes half-duplex. For each website, there should be a chosen unmonitored twin of which the common supersequence is calculated. Whenever the user is about to visit each, their traffic trace is molded into it. In theory, no attack is able to achieve more than 50\% success rate against Walkie-Talkie. Wang \textit{et al.} reported a bandwidth and latency overhead of 31\% and 34\%, respectively, for their model. Deep fingerprinting [36m] obtained 49.7\% accuracy against Walkie-Talkie. 


==> content/perf_tables_color.tex <==


